Measurement of the $t\bar{t}Z$ and $t\bar{t}W$ production cross sections in multilepton final states using 3.2 fb$^{-1}$ of $pp$ collisions at $\sqrt{s}$ = 13 TeV with the ATLAS detector

A measurement of the $t\bar{t}Z$ and $t\bar{t}W$ production cross sections in final states with either two same-charge muons, or three or four leptons (electrons or muons) is presented. The analysis uses a data sample of proton-proton collisions at $\sqrt{s} = 13$ TeV recorded with the ATLAS detector at the Large Hadron Collider in 2015, corresponding to a total integrated luminosity of 3.2 fb$^{-1}$. The inclusive cross sections are extracted using likelihood fits to signal and control regions, resulting in $\sigma_{t\bar{t}Z} = 0.9 \pm 0.3$ pb and $\sigma_{t\bar{t}W} = 1.5 \pm 0.8$ pb, in agreement with the Standard Model predictions.

==> Ackno-Bibtex_2Aug-2016.tex <==
% Acknowledgements for papers with collision data
% Version 2-Aug-2016

% Bibitem entry for the Tier2 facilities reference
%-------------------------------------------------
@Booklet{ATL-GEN-PUB-2016-002,
          author         = "{ATLAS Collaboration}",
          title          = "{ATLAS Computing Acknowledgements
      2016-2017}",
          howpublished   = "{ATL-GEN-PUB-2016-002}",
          url            = "http://cds.cern.ch/record/2202407",
          year           = "2016",
      } 
%----------------------------------------------


